BiosERC: Integrating Biography Speakers Supported by LLMs for ERC Tasks

In the Emotion Recognition in Conversation task, recent investigations have utilized attention mechanisms exploring relationships among utterances from intra- and inter-speakers for modeling emotional interaction between them. However, attributes such as speaker personality traits remain unexplored and present challenges in terms of their applicability to other tasks or compatibility with diverse model architectures. Therefore, this work introduces a novel framework named BiosERC, which investigates speaker characteristics in a conversation. By employing Large Language Models (LLMs), we extract the "biographical information" of the speaker within a conversation as supplementary knowledge injected into the model to classify emotional labels for each utterance. Our proposed method achieved state-of-the-art (SOTA) results on three famous benchmark datasets: IEMOCAP, MELD, and EmoryNLP, demonstrating the effectiveness and generalization of our model and showcasing its potential for adaptation to various conversation analysis tasks. Our source code is available at https://github.com/yingjie7/BiosERC.

==> learning_curver.tex <==
Steps	baseline_min	baseline_max	baseline_avg	bioserc_min	bioserc_max	bioserc_avg	biosattn_min	biosattn_max	biosattn_avg
778	58.39794921875	59.56991958618164	59.16065216064453	55.98782730102539	57.13881587982178	56.75084114074707	56.50459384918213	58.03281307220459	57.02718734741211
1037	59.43125629425049	60.1254358291626	59.918596267700195	58.62678050994873	61.584046363830566	59.88576316833496	60.15866470336914	61.22030448913574	60.81243896484375
1297	59.44133472442627	61.53008270263672	61.20180320739746	59.578850746154785	62.695194244384766	61.80013465881348	59.485647201538086	61.27329349517822	60.947288513183594
1556	60.344767570495605	61.816659927368164	61.19702911376953	61.38814353942871	63.08159923553467	62.59757423400879	60.31164264678955	61.846675872802734	61.38675498962402
1816	61.979007720947266	62.708930015563965	62.21635818481445	62.36879062652588	63.33630657196045	63.06816864013672	60.07465648651123	62.41869831085205	61.64267539978027
2075	61.62794589996338	62.42567253112793	61.97010612487793	62.99513053894043	64.22224712371826	63.58481216430664	60.507205963134766	62.395599365234375	61.68050193786621
2335	61.078166007995605	62.64348316192627	62.1339225769043	61.608673095703125	63.15179443359375	62.70804405212402	61.508056640625	62.979342460632324	62.895050048828125
2594	59.914992332458496	62.02158260345459	61.71923637390137	62.32487964630127	63.717247009277344	63.3388671875	60.906487464904785	62.951172828674316	61.446937561035156
2854	61.53048896789551	63.27760887145996	62.834489822387695	62.71117115020752	64.51401138305664	63.56062889099121	60.56707000732422	62.77161693572998	62.29022026062012
3113	62.172425270080566	63.045448303222656	62.444976806640625	62.22006893157959	63.99636936187744	63.337440490722656	62.529738426208496	63.87174987792969	63.62044334411621
3373	61.78211498260498	63.22984790802002	62.486419677734375	62.39285659790039	63.683043479919434	63.31690216064453	62.002071380615234	63.09051704406738	62.397939682006836
3632	61.48935890197754	63.96185493469238	63.290632247924805	63.339118003845215	64.41019058227539	64.05400466918945	61.58811855316162	63.12370204925537	62.71066856384277
3892	62.55818176269531	63.990437507629395	63.56454658508301	63.473886489868164	64.95990180969238	64.07418823242188	61.2805700302124	63.65809726715088	62.40171813964844
4151	62.77813529968262	63.59912109375	63.09753608703613	64.12223815917969	64.70345878601074	64.31932830810547	62.71206474304199	63.720895767211914	63.336957931518555
4411	62.549367904663086	63.840697288513184	63.36209487915039	63.446743965148926	64.41458892822266	63.6177978515625	62.931260108947754	64.4666805267334	63.47283935546875
4670	63.98832035064697	64.27227210998535	64.09623718261719	64.26859664916992	65.7442855834961	64.5689811706543	63.6018180847168	64.05327415466309	63.789459228515625
4930	63.222177505493164	64.17227554321289	63.792633056640625	63.633172035217285	64.51303482055664	64.18290710449219	62.744513511657715	64.74579334259033	63.38474464416504
5189	63.828980445861816	64.45481300354004	63.92754936218262	63.914655685424805	64.6348991394043	64.33676528930664	62.527177810668945	64.33550262451172	63.3782958984375
5449	63.42504596710205	64.99135398864746	64.36872100830078	64.00716781616211	64.72027397155762	64.65189361572266	63.421579360961914	64.31902885437012	64.08442687988281
5708	63.449222564697266	64.43700408935547	63.77095031738281	64.05006790161133	64.98854064941406	64.34612274169922	63.974257469177246	65.16458320617676	64.75672912597656
5968	62.829423904418945	63.834824562072754	63.348785400390625	63.90903854370117	65.3494873046875	64.8358154296875	63.737406730651855	64.89301872253418	64.02867889404297
6227	64.11294746398926	64.68787574768066	64.30896377563477	64.48900604248047	65.36057472229004	64.6807975769043	63.99704456329346	65.23608207702637	64.80081558227539
6487	64.38646697998047	64.89217948913574	64.60176467895508	64.14375877380371	65.46854209899902	64.90152359008789	63.39182949066162	64.95145606994629	64.38336944580078
6746	64.14418411254883	65.11156463623047	64.57315063476562	63.54632759094238	66.17622184753418	64.99838638305664	64.89057540893555	65.32742118835449	65.21254348754883
7006	63.80726432800293	64.60358428955078	63.90779495239258	64.56447792053223	65.84383201599121	65.4481201171875	64.87555694580078	65.97433471679688	65.14188766479492
7265	64.0272912979126	65.17126846313477	64.36843872070312	64.2807388305664	66.1313362121582	65.17136001586914	64.36225700378418	65.65324783325195	65.24351119995117
7525	63.74251174926758	64.98984336853027	64.09530639648438	64.61891174316406	66.27456283569336	65.26762771606445	64.37999153137207	65.06266975402832	64.69307708740234
7784	63.807074546813965	65.24443244934082	64.77939987182617	64.92217254638672	66.05644798278809	65.49745178222656	64.62792015075684	65.23981857299805	64.91856002807617


==> length_analysis_processed.tex <==
idx	length	baseline_min	baseline_max	baseline_avg	bioserc_min	bioserc_max	bioserc_avg
1	[0-5)	62.552499999999995	65.6175	63.8	65.2225	69.525	68.38999999999999
2	[5-10)	66.29249999999999	68.14500000000001	67.86	67.4875	69.8875	68.725
3	[10-15)	65.2475	66.6725	65.63	66.36500000000001	68.19999999999999	67.59
4	[15-20)	64.42750000000001	65.9025	65.41	64.875	67.5	66.125
5	[20-)	66.3375	68.2225	67.18	66.08250000000001	67.5925	67.055

